MS-Shift: An Analysis of MS MARCO Distribution Shifts on Neural Retrieval

Pre-trained Language Models have recently emerged in Information Retrieval as providing the backbone of a new generation of neural systems that outperform traditional methods on a variety of tasks. However, it is still unclear to what extent such approaches generalize in zero-shot conditions. The recent BEIR benchmark provides partial answers to this question by comparing models on datasets and tasks that differ from the training conditions. We aim to address the same question by comparing models under more explicit distribution shifts. To this end, we build three query-based distribution shifts within MS MARCO (query-semantic, query-intent, query-length), which are used to evaluate the three main families of neural retrievers based on BERT: sparse, dense, and late-interaction -- as well as a monoBERT re-ranker. We further analyse the performance drops between the train and test query distributions. In particular, we experiment with two generalization indicators: the first one based on train/test query vocabulary overlap, and the second based on representations of a trained bi-encoder. Intuitively, those indicators verify that the further away the test set is from the train one, the worse the drop in performance. We also show that models respond differently to the shifts -- dense approaches being the most impacted. Overall, our study demonstrates that it is possible to design more controllable distribution shifts as a tool to better understand generalization of IR models. Finally, we release the MS MARCO query subsets, which provide an additional resource to benchmark zero-shot transfer in Information Retrieval.

==> general_msmarco.tex <==
\begin{table}[t]
\begin{center}
    \caption{Avg performances on the original MSMARCO/TREC datasets. Models were subject to the shifts at training time. \textit{All} means using the whole/standard training set.}
    \label{tab:all}
    \begin{tabular}{l | c | c c c c}
        \toprule
        Models & Training & \multicolumn{2}{c}{MSMARCO dev} & \multicolumn{2}{c}{TREC DL 2019} \\ 
        & subsets& MRR@10 & R@1k & NDCG@10 & R@1k \\ \midrule
        Siamese & Topics & 0.274 & 0.921 & 0.592 & 0.709 \\ 
         & WH & 0.251 &  0.908 & 0.550 & 0.685 \\ 
         & Length & 0.290& 0.931 & 0.609 & 0.719 \\ 
         & All  & 0.311 & 0.947 & 0.641 & 0.741 \\ \midrule
        SPLADE & Topics & 0.312 & 0.950 & 0.650& 0.779 \\ 
         & WH & 0.297 & 0.944 & 0.632 & 0.790 \\ 
         & Length & 0.314& 0.953 & 0.667 & 0.788 \\  
          & All & 0.344 & 0.965 & 0.678 & 0.799 \\ \midrule
        ColBERT & Topics & \textbf{0.337}& \textbf{0.958} & \textbf{0.682} & \textbf{0.810} \\ 
         & WH & \textbf{0.331}& \textbf{0.961} & \textbf{0.677} & \textbf{0.829}\\ 
         & Length & \textbf{0.343} & \textbf{0.964} & \textbf{0.710} & \textbf{0.827} \\
          & All & \textbf{0.356} & \textbf{0.970} & \textbf{0.692} & \textbf{0.832} \\ 
        \bottomrule
    \end{tabular}   
\end{center}
\end{table}

% MRR@10 (Siam, SPLADE, ColBERT)
% 0.921 0.754 - -
% 0.816 0.8 0.876 -
% 0.931 0.943 0.953 0.921

==> t1.tex <==

\begin{table}[h]
\begin{center}
    \caption{Evaluation of SPLADE on Query Topics. Each cluster has a train/eval split to enable evaluation on seen/unseen clusters. Rows correspond to training, cols to evaluation.} %Underlined are the lower performances on a given cluster.}
    \label{tab:rotation}
    \begin{tabular}{l | c c c c c}
        \toprule
        MRR@10 & $C_0^e$ & $C_1^e$ & $C_2^e$ & $C_3^e$ & $C_4^e$  \\ \midrule
        $\overline{C_0}^t$ & \underline{0.345} &	0.386 &	0.303 &	0.255& 	\underline{0.242} \\ 
        $\overline{C_1}^t$ &0.360 &	\underline{0.339} &	0.314 &	0.270 &	0.258 \\ 
        $\overline{C_2}^t$ & 0.369 &	0.381 &	\underline{0.302} &	0.268 &	0.256 \\ 
        $\overline{C_3}^t$ & 0.371 &	0.395 &	0.317 &	\underline{0.246} &	0.246 \\ 
        $\overline{C_4}^t$ & 0.372 &	0.384 &	0.315 &	0.256 &	0.247 \\ \midrule
        Avg In & 0.368 & 0.387 & 0.312  & 0.262 & 0.250 \\
        Rel Loss Out & 6.3\% & 12.2\% & 3.2\% & 6.4\% & 1.4\% \\
        \bottomrule
    \end{tabular}   
\end{center}
\end{table}

==> t3.tex <==
\begin{table}[h]
\begin{center}
    \caption{Evaluation of Short and Long queries when trained on short and long queries separately.}
    \label{tab:short}
    \begin{tabular}{l | c | c c}
        \toprule
        Models &  & short & long \\ \midrule
        Siamese & Avg In & 0.340 &0.271	  \\ 
        & Rel Loss Out & 12.5\% & 7.0\% \\ \midrule
        ColBERT & Avg In &  \textbf{0.382} &  \textbf{0.320}   \\ 
        & Rel Loss Out & 6.0\% & \textbf{2.2\%} \\ \midrule
        SPLADE & Avg In & 0.349 &0.303	  \\ 
        & Rel Loss Out & 3.9\% & 10.4\% \\ 
        +Adv & Avg In &  0.350 & 0.307  \\ 
        & Rel Loss Out & \textbf{1.0\%} & 11.1\% \\
        \bottomrule
    \end{tabular}   
\end{center}
\end{table}


%\begin{table}[h]
%    \caption{Evaluation of Short and Long queries when trained on short and long queries separately.}
%    \label{tab:short}
%    \begin{tabular}{l | c | c c}
%        \toprule
%        Models & Train ($\downarrow$) Eval ($\rightarrow$) & short & long \\ \midrule
%        Siamese & short & 0.340 &0.252	  \\ 
%        & long & 0.298 &0.271	 \\ 
%        & Rel Loss Out & 12.5\% & 07.0\% \\ \midrule
%        ColBERT & short &  \textbf{0.382} &  \textbf{0.313}   \\ 
%        & long &   \textbf{0.359} & \textbf{0.320}  	 \\ 
%        & Rel Loss Out & 06.0\% & \textbf{02.2\%} \\ \midrule
%        SPLADE & short & 0.349 &0.272	  \\ 
%        & long & 0.336 &0.303	 \\ 
%        & Rel Loss Out & 03.9\% & 10.4\% \\ 
%        +Adv & short &  0.350 & 0.273  \\ 
%        & long &   0.346 & 0.307	 \\ 
%        & Rel Loss Out & \textbf{01.0\%} & 11.1\% \\
%        \bottomrule
%    \end{tabular}   
%\end{table}
